Learning from Convolution-based Unlearnable Datasets

The construction of large datasets for deep learning has raised concerns regarding unauthorized use of online data, leading to increased interest in protecting data from third-parties who want to use it for training. The Convolution-based Unlearnable DAtaset (CUDA) method aims to make data unlearnable by applying class-wise blurs to every image in the dataset so that neural networks learn relations between blur kernels and labels, as opposed to informative features for classifying clean data. In this work, we evaluate whether CUDA data remains unlearnable after image sharpening and frequency filtering, finding that this combination of simple transforms improves the utility of CUDA data for training. In particular, we observe a substantial increase in test accuracy over adversarial training for models trained with CUDA unlearnable data from CIFAR-10, CIFAR-100, and ImageNet-100. In training models to high accuracy using unlearnable data, we underscore the need for ongoing refinement in data poisoning techniques to ensure data privacy. Our method opens new avenues for enhancing the robustness of unlearnable datasets by highlighting that simple methods such as sharpening and frequency filtering are capable of breaking convolution-based unlearnable datasets.

==> figures/blur_parameter_analysis.tex <==
\begin{figure}
\centering
\resizebox{8.3cm}{!}{
\begin{tikzpicture}
\begin{axis}[
    xlabel={Blur Parameter $p_b$},
    ylabel={CIFAR-10 Test Accuracy},
    xmin=0.1, xmax=0.9,
    ymin=0, ymax=100,
    xtick={0.1,0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9},
    ytick={0,10,20,30,40,50,60,70,80,90,100},
    legend pos=north east, 
    legend style={nodes={scale=0.7, transform shape}}, % scale=0.7
    ymajorgrids=true,
    grid style=dashed,
    every axis plot/.append style={no markers, very thick}
]

%
% Input data for lines
%
\input{figures/data/random_blurs}
\input{figures/data/nonrandom_blurs}
\input{figures/data/clean_blurs}

%
%
% 
% \node[anchor=north west] at (rel axis cs:0,1) {\textbf{(a)}};

% mark best DFR checkpoint with star
%\node[star, star points=5, star point ratio=2.25, draw=yellow, fill=yellow, inner sep=1.3pt] at (axis cs:53,69.99) {};

\legend{Random Sharpening Kernel, Sharpening Kernel, CUDA}

\end{axis}
\end{tikzpicture}
}
\caption{This analysis uses our best recipe for learning from CUDA on the CIFAR-10 dataset: random sharpening kernel with center 2.5, and JPEG compression with quality 10. We also include test accuracies for a standard sharpening kernel with JPEG 10. The yellow dotted line visualizes the accuracy for images affected by only CUDA.}
\label{fig:blur_graph}
\end{figure}

==> figures/data/clean_blurs.tex <==
\addplot[yellow, densely dashed]
coordinates{
(0.1, 53.076)
(0.2, 34.276)
(0.3, 22.24)
(0.4, 17.84)
(0.5, 15.306)
(0.6, 15.244)
(0.7, 15.268)
(0.8, 15.16)
(0.9, 14.04)
};

==> figures/data/nonrandom_blurs.tex <==
\addplot[violet, densely dashed]
coordinates{
(0.1, 77.28)
(0.2, 71.67)
(0.3, 57.38)
(0.4, 52.23)
(0.5, 51.14)
(0.6, 47.08)
(0.7, 46.20)
(0.8, 46.74)
(0.9, 47.44)
};

==> figures/data/random_blurs.tex <==
\addplot[violet]
coordinates{
(0.1, 85.54)
(0.2, 79.59)
(0.3, 71.02)
(0.4, 62.91)
(0.5, 59.05)
(0.6, 58.21)
(0.7, 57.44)
(0.8, 59.39)
(0.9, 58.35)
};

==> figures/dct_analysis.tex <==
\begin{figure}
\centering
\resizebox{8.3cm}{!}{
\begin{tikzpicture}
\begin{axis}[
    xlabel={Percentage of Kept DCT Frequencies},
    ylabel={CIFAR-10 Test Accuracy},
    xmin=10, xmax=100,
    ymin=0, ymax=100,
    xtick={10,20,30,40,50,60,70,80,90,100},
    ytick={0,10,20,30,40,50,60,70,80,90,100},
    legend pos=north east, 
    legend style={nodes={scale=0.7, transform shape}}, % scale=0.7
    ymajorgrids=true,
    grid style=dashed,
    every axis plot/.append style={no markers, very thick}
]

%
% Input data for lines
%
\input{figures/dct_analysis/dct_on_clean}
\input{figures/dct_analysis/dct_on_just_cuda}
\input{figures/dct_analysis/dct_on_rsk_cuda}
\input{figures/dct_analysis/dct_on_jpeg_cuda}
\input{figures/dct_analysis/dct_on_rsk_jpeg_cuda}
%
%
% 
% \node[anchor=north west] at (rel axis cs:0,1) {\textbf{(a)}};

% mark best DFR checkpoint with star
%\node[star, star points=5, star point ratio=2.25, draw=yellow, fill=yellow, inner sep=1.3pt] at (axis cs:53,69.99) {};

\legend{Baseline, CUDA, CUDA + RSK, CUDA + JPEG, CUDA + RSK + JPG}

\end{axis}
\end{tikzpicture}
}
\caption{TODO}
\label{fig:dct_graph}
\end{figure}

==> figures/transforms.tex <==
\begin{figure*}
    \centering
    \resizebox{8cm}{!}{
        \includegraphics{figures/images/transform_comparison.png}
    }
    \caption{\textbf{Sharpening kernels make CUDA images more clear.} The top row contain a clean image and transforms of the clean image. The bottom row contains a CUDA image and the transforms of the CUDA image. \textbf{JPEG(10)} refers to JPEG compression with quality 10, the lowest possible, \textbf{Sharpen(2.5)} refers to the nonrandom sharpening kernel with center 2.5, and \textbf{Random(2.5)} refers to our random sharpening kernel with center 2.5. From Table~\ref{table:jpeg_table}, our test accuracies are surprisingly high, considering how malformed the images look when our transforms are applied. }
    \label{fig:comparison}
\end{figure*}

==> tables/sharpening_table.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|ccc}
\toprule
Transform     & CIFAR-10 & CIFAR100 & ImageNet-100 \\ \midrule
Sharpen (2.5) & 26.72\%  & 28.29\%  & 2.78\%       \\
Random (2.5)  & 29.94\%  & 33.52\%  & 5.56\%      
\end{tabular}
\vspace{0.5cm}
\caption{This table shows a breakdown of our sharpening kernels, and the test accuracies for each.  Both experiments use a blur parameter $p_b$ of $0.3$. See Section 4 for experiment details. }
\label{table:sharpening_table}
\end{table}




